Everything old is new again: Quoted Domain Specific Languages

We describe a new approach to domain specific languages (DSLs), called Quoted DSLs (QDSLs), that resurrects two old ideas: quotation, from McCarthy's Lisp of 1960, and the subformula property, from Gentzen's natural deduction of 1935. Quoted terms allow the DSL to share the syntax and type system of the host language. Normalising quoted terms ensures the subformula property, which guarantees that one can use higher-order types in the source while guaranteeing first-order types in the target, and enables using types to guide fusion. We test our ideas by re-implementing Feldspar, which was originally implemented as an Embedded DSL (EDSL), as a QDSL; and we compare the QDSL and EDSL variants.

==> formalism.tex <==
%% Types
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\arrow}[2]{#1\rightarrow#2}
\newcommand{\product}[2]{#1\times#2}
\newcommand{\coproduct}[2]{#1+#2}
\newcommand{\rec}[2]{\mu#1.#2}

%% Expressions
\newcommand{\key}{\mathbf}

\newcommand{\app}{\;}

\newcommand{\expvar}[1]{#1}
\newcommand{\expconst}[2]{#1~#2}
\newcommand{\expunit}{()}
\newcommand{\expabs}[3]{\lambda#1.\,#3}
\newcommand{\expapp}[2]{#1 \app #2}
\newcommand{\explet}[3]{\key{let}\ #1=#2\ \key{in}\ #3}
\newcommand{\exppair}[2]{(#1, #2)}
\newcommand{\expfst}[1]{\key{fst}~#1}
\newcommand{\expsnd}[1]{\key{snd}~#1}
\newcommand{\expinl}[2]{\key{inl}~#1}
\newcommand{\expinr}[2]{\key{inr}~#2}
\newcommand{\expcase}[5]
  {\key{case}\ #1\ \key{of}\ \{\key{inl}\ #2.\,#3;\; \key{inr}\ #4.\,#5\}}

%% Meta language stuff
\newcommand{\subst}[3]{#1[#2:=#3]}
\newcommand{\fv}[1]{\mathit{FV}(#1)}
\newcommand{\rewrite}[1]{\mathbin{\mapsto_{#1}}}
\newcommand{\hole}{[~]}

%% Typing
\newcommand{\intro}{\mathcal{I}}
\newcommand{\elim}{\mathcal{E}}
\newcommand{\inference}[3]{\infer[\mathsf{#2}]{#3}{#1}}

\newcommand{\figterm}{
\begin{figure*}[t]
\[
\begin{array}{l@@{\quad}rcl}
\text{Types} & A,B,C & ::=&
% \one
  \iota           \mid
  \arrow{A}{B}    \mid
  \product{A}{B}  \mid
  \coproduct{A}{B}
\\[1ex]
\text{Terms} & L,M,N & ::= &
  \expvar{x}              	\mid
  \expconst{c}{\overline{M}}	\mid
  \expabs{x}{A}{N}              \mid
  \expapp{L}{M}                 \mid
  \explet{x}{M}{N}              \mid
  \exppair{M}{N}                \mid
  \expfst{L}                   	\mid
  \expsnd{L}                    \mid \\&&&
  \expinl{M}{\tm{B}}		\mid
  \expinr{\tm{A}}{N}           	\mid
  \expcase{L}{x}{M}{y}{N}
\\[1ex]
\text{Values} & V,W & ::= &
  \expvar{x}       \mid
  \expabs{x}{A}{N} \mid
  \exppair{V}{W}   \mid
  \expinl{V}{B}    \mid
  \expinr{A}{W}
% \\[1ex]
% \text{Non-Values} & P & ::= &
%   \expconst{c}{\overline{M}}  \mid
%   \expapp{L}{M}               \mid
%   \explet{x}{M}{N}            \mid
%   \exppair{P}{N}              \mid
%   \exppair{V}{P}              \mid
%   \expfst{P}                  \mid
%   \expsnd{P}                  \mid \\&&&
%   \expinl{P}{\tm{B}}          \mid
%   \expinr{\tm{A}}{P}          \mid
%   \expcase{L}{x}{M}{y}{N}
\end{array}
\]

\caption{Types and Terms}
\label{fig:term}
\end{figure*}
}

\newcommand{\figtyping}{
\begin{figure*}[h]
\[
\begin{array}{@@{}ll@@{}}
\fbox{$\Gamma \vdash M:A$}
\\~\\
\inference
{x:A \in \Gamma}
{\mathbf{Ax}}
{
  \Gamma \vdash x:A
}
&
\inference
{}
{\one}
{
   \Gamma \vdash \expunit:\one
}
\\~\\
\inference
{
  \Gamma, x:A \vdash N:B
}
{{\to}\intro}
{
  \Gamma \vdash \expabs{x}{A}{N}:\arrow{A}{B}
}
&
\inference
{
  \Gamma \vdash L:\arrow{A}{B}
& \Gamma \vdash M:A
}
{{\to}\elim}
{
  \Gamma \vdash \expapp{L}{M}:B
}
\\~\\
\inference
{
  \Gamma \vdash M:A
  &
  \Gamma, x:A \vdash N:B
}
{\mathbf{let}}
{
  \Gamma \vdash \explet{x}{M}{N}:B
}
&
\inference
{
  \Gamma \vdash M:A
  &
  \Gamma \vdash N:B
}
{{\times}\intro}
{
  \Gamma \vdash \exppair{M}{N}:\product{A}{B}
}
\\~\\
\inference
{
  \Gamma \vdash L:\product{A}{B}
}
{{\times}\elim_1}
{
  \Gamma \vdash \expfst{L}:A
}
&
\inference
{
  \Gamma \vdash L:\product{A}{B}
}
{{\times}\elim_2}
{
  \Gamma \vdash \expsnd{L}:B
}
\\~\\
\inference
{
  \Gamma \vdash M:A
}
{{+}\intro_1}
{
  \Gamma \vdash \expinl{M}{B}:\coproduct{A}{B}
}
&
\inference
{
  \Gamma \vdash N:B
}
{{+}\intro_2}
{
  \Gamma \vdash \expinr{A}{N}:\coproduct{A}{B}
}
\\~\\
\inference
{
  \Gamma \vdash L:\coproduct{A}{B}
&
  \Gamma, x:A \vdash M:C
&
  \Gamma, y:B \vdash N:C
}
{{+}\elim}
{
  \Gamma \vdash \expcase{L}{x}{M}{y}{N}:C
}
\end{array}
\]
\caption{Typing Rules}
\label{fig:typing}
\end{figure*}
}

\newcommand{\fignf}{
\begin{figure*}[t]
\[
\begin{array}{l@@{\quad}rcl}
\text{Neutral Forms}
  & Q & ::= & \expapp{x}{W}
         \mid \expconst{c}{\overline{W}}
         \mid \expapp{Q}{W}
         \mid \expfst{x}
         \mid \expsnd{x}
\\[1ex]
\text{Normal Values}
  & V,W & ::= & \expvar{x}
           \mid \expabs{x}{A}{N}
           \mid \exppair{V}{W}
           \mid \expinl{V}{B}
           \mid \expinr{A}{W}
\\[1ex]
\text{Normal Forms}
  & N,M & ::= & Q
          \mid  V
          \mid \expcase{z}{x}{N}{y}{M}
          \mid \explet{x}{Q}{N}
\\
\end{array}
\]
\caption{Normal Forms}
\label{fig:nf}
\end{figure*}
}

\newcommand{\fignorm}{
\begin{figure*}[t]
Phase 1 (let-insertion)
\[
  \begin{array}{lcl}
   F &\mathbin{::=}&
%      c \app \overline{V} \app \hole \app \overline{N} \mid
       \expapp{\hole}{M}                                \mid
       \expapp{V}{\hole}                                \mid
       \exppair{\hole}{M}                               \mid
       \exppair{V}{\hole}                               \mid
       \expfst{\hole}                                   \mid
       \expsnd{\hole}                                   \mid % \\ &&
       \expinl{\hole}{B}                                \mid
       \expinr{A}{\hole}                                \mid
       \expcase{\hole}{x}{M}{y}{N} \\
 \end{array}
\]%
\[
\begin{array}{lllll}
(\mathit{let})
& F[M]
& \rewrite{1}
& \explet{x}{M}{F[x]},
& \text{$x$ fresh, $M$ not a value}
\end{array}
\]

\vspace{2ex}

Phase 2 (symbolic evaluation)
\[
G \mathbin{::=}
    %\expapp{\hole}{V} \mid
    \explet{x}{\hole}{N}
\]
\[
\begin{array}{lllll}
%% SL: given that G now only has one case we could use the
%% explicit versions of the $\kappa$-rules, but actually I think
%% this version is harder to read.
%%
%% (\kappa.{\mathit{let}})
%% & \explet{y}{\explet{x}{L}{M}}{N}
%% & \rewrite{2}
%% & \explet{x}{L}{\explet{y}{M}{N}},
%% & x \notin \fv{M} \\
%%
%% (\kappa.{\mathit{case}})
%% & \explet{z}{\expcase{L}{x}{M}{y}{M'}}{N}
%% & \rewrite{2}
%% & \expcase{L}{x}{\explet{z}{M}{N}}{y}{\explet{z}{M'}{N}},
%% & x,y \notin \fv{N} \\

(\kappa.{\mathit{let}})
& G[\explet{x}{M}{N}]
& \rewrite{2}
& \explet{x}{M}{G[N]},
& x \notin \fv{G} \\

(\kappa.{\mathit{case}})
& G[\expcase{V}{x}{M}{y}{N}]
& \rewrite{2}
& \expcase{V}{x}{G[M]}{y}{G[N]},
& x,y \notin \fv{G} \\

% (\kappa.{\mathit{case}})
% & G[\expcase{z}{x}{M}{y}{N}] & \rewrite{2}\\
% \multicolumn{3}{@@{}l@@{}}
% {\qquad\qquad\qquad\quad \expcase{z}{x}{G[M]}{y}{G[N]},} & \quad x,y \notin \fv{G} \\[1ex]

(\beta.{\rightarrow})
& \expapp{(\expabs{x}{A}{N})}{V}
& \rewrite{2}
& \subst{N}{x}{V} \\

(\beta.{\times_1})
& \expfst{\exppair{V}{W}}
& \rewrite{2}
& V \\

(\beta.{\times_2})
& \expsnd{\exppair{V}{W}}
& \rewrite{2}
& W \\

(\beta.{+_1})
& \expcase{(\expinl{V}{B})}{x}{M}{y}{N}
& \rewrite{2}
& \subst{M}{x}{V} \\

(\beta.{+_2})
& \expcase{(\expinr{A}{W})}{x}{M}{y}{N}
& \rewrite{2}
& \subst{N}{y}{W} \\

(\beta.{\mathit{let}})
& \explet{x}{V}{N}
& \rewrite{2}
& \subst{N}{x}{V} \\
\end{array}
\]

\vspace{2ex}

Phase 3 (garbage collection)
\[
\begin{array}[t]{@@{}llll@@{\quad}l@@{}}

(\mathit{need})
& \explet{x}{M}{N}
& \rewrite{3}
& N,
& x \notin \fv{N}\\
%% & \subst{N}{x}{P},
%% & Count(x,N) < 2 \\
\end{array}
\]

\caption{Normalisation Rules}
\label{fig:norm}
\end{figure*}
}

